Making Classic GNNs Strong Baselines Across Varying Homophily: A Smoothness-Generalization Perspective

Graph Neural Networks (GNNs) have achieved great success but are often considered to be challenged by varying levels of homophily in graphs. Recent \textit{empirical} studies have surprisingly shown that homophilic GNNs can perform well across datasets of different homophily levels with proper hyperparameter tuning, but the underlying theory and effective architectures remain unclear. To advance GNN universality across varying homophily, we theoretically revisit GNN message passing and uncover a novel \textit{smoothness-generalization dilemma}, where increasing hops inevitably enhances smoothness at the cost of generalization. This dilemma hinders learning in high-order homophilic neighborhoods and all heterophilic ones, where generalization is critical due to complex neighborhood class distributions that are sensitive to shifts induced by noise or sparsity. To address this, we introduce the Inceptive Graph Neural Network (IGNN) built on three simple yet effective design principles, which alleviate the dilemma by enabling distinct hop-wise generalization alongside improved overall generalization with adaptive smoothness. Benchmarking against 30 baselines demonstrates IGNN's superiority and reveals notable universality in certain homophilic GNN variants. Our code and datasets are available at \href{https://github.com/galogm/IGNN}{https://github.com/galogm/IGNN}.

==> proofs/equal.tex <==
\begin{proof}[Proof of \cref{prop:equal}]
\label{prf:equal}
    A concatenative \model with a single transformation layer in both \SN and \RN can be expressed as:
    \begin{equation}
        \mathbf{H}
        =\sigma\left( (\underset{k=0}{\overset{K}{||}}\sigma(\widehat{\mathbf{A}}^k \mathbf{X} \mathbf{W}^{(k)}))\mathbf{W} \right)
        =\sigma\left( \sum_{k=0}^K \sigma(\widehat{\mathbf{A}}^k \mathbf{X} \mathbf{W}^{(k)})\mathbf{W}_k \right),
        \text{where } \mathbf{W}=\left[\begin{smallmatrix}\mathbf{W}_0\\\cdots\\\mathbf{W}_k\\\cdots\\\mathbf{W}_K\end{smallmatrix}\right]\in \mathbb{R}^{KF\times F'}.
    \end{equation}
    Since $\sigma(\cdot)$ is non-parametric, the following holds:
    \begin{equation}
        \mathbf{H}
        =\sigma\left( \sum_{k=0}^K \sigma(\widehat{\mathbf{A}}^k \mathbf{X} \mathbf{W}^{(k)})\mathbf{W}_k \right)
        = \sum_{k=0}^K \sigma\left(\sigma(\widehat{\mathbf{A}}^k \mathbf{X} \mathbf{W}^{(k)})\mathbf{W}_k \right).
    \end{equation}
    Rearranging the terms, we also have: $\mathbf{H}= \sigma\left(\sigma( (\sum_{k=0}^K \widehat{\mathbf{A}}^k \mathbf{X}) \mathbf{W}^{(k)})\mathbf{W}_k \right).$
    This representation aligns with either (i) the format of two transformation layers in \SN and no transformation layers in \RN, or (ii) two transformation layers in \RN and no transformation layers in \SN.
    Therefore, a single transformation layer in \SN is equivalent to a single transformation layer in \RN.
\end{proof}

==> sections/theorems.tex <==
\section{Theoretical Analysis}

\label{sec:theorems}

\subsection{The Information Loss of the Message Passing}

In this section, we theoretically demonstrate the following points:
(1) Once multi-hop neighborhood mixing occurs, information loss at the $k$-th hop becomes inevitable, making it impossible to recover or discriminate through post-processing.
(2) The rate of information loss in the message-passing framework is faster compared to embedding each hop neighborhood individually.

If denoting the $k$-hop neighborhood as $\widehat{\mathbf{A}}^k$, in the MP process of GCN, obtaining the information of $\widehat{\mathbf{A}}^k$ requires $k$ rounds of MP to get its representation.
However, instead of performing $k$ rounds of MP, one can alternatively gather the information directly from the exact $k$-hop neighborhood in a single step.
The following theorem demonstrates that the former approach results in greater information loss compared to the latter.
\begin{theorem}
\label{tm:infoloss}
Given a graph $\mathcal{G}(\mathbf{X},\mathbf{A})$, denote the representation of the $k$-hop neighborhood by $k$ rounds of message passing on $\widehat{\mathbf{A}}$ as 
$\mathbf{H}^{(k)}_{\widehat{\mathbf{A}}} = \sigma(\widehat{\mathbf{A}}\mathbf{H}^{(k-1)}\mathbf{W}^{(k)})$, 
and the representation obtained by directly gathering from ${\widehat{\mathbf{A}}^k}$ as
$\mathbf{H}^{(1)}_{\widehat{\mathbf{A}}^k} = \sigma(\widehat{\mathbf{A}}^k\mathbf{X}\mathbf{W}^{(1)})$.
$\mathbf{H}^{(k)}_{\widehat{\mathbf{A}}}$ experiences more information loss from  $\mathbf{X}$ than $\mathbf{H}^{(1)}_{\widehat{\mathbf{A}}^k}$, as the distances from each representation to $\mathcal{M}$ satisfy: $d_\mathcal{M}(\mathbf{H}_{\widehat{\mathbf{A}}}^{(k)})\le s^{k-1}d_\mathcal{M}(\mathbf{H}^{(1)}_{\widehat{\mathbf{A}}^k})$.
\end{theorem}
Since this subspace $\mathcal{M}$ represents the convergence state where the least amount of information is retained~\citep{subspace}, we can infer that a smaller distance indicates that the hidden representation $d_\mathcal{M}(\mathbf{H}_{\widehat{\mathbf{A}}}^{(k)})$  retains less information than $d_\mathcal{M}(\mathbf{H}^{(1)}_{\widehat{\mathbf{A}}^k})$ .


\begin{theorem}
\label{tm:dmspeed}
Given a graph $\mathcal{G}(\mathbf{X},\mathbf{A})$, denote the representation of the $k$-hop neighborhood by $k$ rounds of message passing on $\widehat{\mathbf{A}}$ as 
$\mathbf{H}^{(k)}_{\widehat{\mathbf{A}}} = \sigma(\widehat{\mathbf{A}}\mathbf{H}^{(k-1)}\mathbf{W}^{(k)})$, 
and the representation obtained by directly gathering from ${\widehat{\mathbf{A}}^k}$ as
$\mathbf{H}^{(1)}_{\widehat{\mathbf{A}}^k} = \sigma(\widehat{\mathbf{A}}^k\mathbf{X}\mathbf{W}^{(1)})$.
The upper bound of the speed $\mathbf{H}^{(k)}_{\widehat{\mathbf{A}}}$ approaches $\mathcal{M}$ denoting as $\mathbf{H}^{(k)}_{\widehat{\mathbf{A}}}/\mathbf{H}^{(k-1)}_{\widehat{\mathbf{A}}}$ is smaller than that of the speed $\mathbf{H}^{(1)}_{\widehat{\mathbf{A}}^k}$ denoting as $\mathbf{H}^{(1)}_{\widehat{\mathbf{A}}^k}/\mathbf{H}^{(1)}_{\widehat{\mathbf{A}}^{(k-1)}}$.
\end{theorem}


==> tabs/nrl-f.tex <==
\begin{table*}[t]
  \centering
  
    \caption{
    Abalation of different \RN Funtions.
    \textit{None} means only non-parametric concatenation.
    \textit{Concat} means concatenation followed by a learnable transformation.
    \textit{Mean-/Sum-/Max-Set} means Deepsets-like set embedding methods, i.e., Mean-/Sum-/Max-Pooling followed by a learnable transformation.
    }
  \resizebox{\textwidth}{!}{
    \begin{tabular}{c|cccccccccc}

      \toprule[1pt]
      \textbf{REL} & \textbf{actor}      & \textbf{blogcatalog} & \textbf{flickr} & \textbf{Roman-E}    & \textbf{squirrel}   & \textbf{chameleon}  & \textbf{amazon-R} & \textbf{pubmed}     & \textbf{photo}      & \textbf{wikics}     \\
      \midrule[0.8pt]
      \textbf{None}     & 36.76±1.00          & 96.06±0.68           & 91.81±0.58          &81.56±0.57 & 42.13±1.99          & 44.66±3.46          & 52.47±0.95     & \textbf{90.29±0.50}          & 95.53±0.43 & 85.59±0.79          \\
      \textbf{Concat}   & \textbf{38.71±1.00}          &\textbf{97.13±0.21} & 92.16±0.66          &85.19±0.53 & \textbf{43.42±1.66} & 44.33±4.57          & \textbf{53.01±0.77}          & 90.23±0.50          & \textbf{95.75±0.38}          & 85.97±0.64          \\
      \textbf{LSTM}     & 37.20±1.27          & 96.38±0.39           & \textbf{93.23±0.61} &\textbf{86.07±0.60} & 41.21±2.84          & 46.52±3.46          & 51.43±0.95              & 90.27±0.72          & 95.41±0.46          & 85.57±0.48          \\
      \textbf{Mean-Set}     & 37.54±1.96          & 96.26±0.41           & 91.88±0.66          &84.80±0.69 & 42.81±1.73          & 44.55±5.04          & 51.99±0.85              & 90.25±0.51 & 95.46±0.47          & 85.95±0.67          \\
      \textbf{Sum-Set}      & 37.76±1.92          & 96.32±0.54           & 91.93±0.61          &84.84±0.65 & 43.26±1.86          & 45.39±4.25          & 51.85±1.08              & 90.25±0.43          & 95.37±0.48          & 85.89±0.64          \\
      \textbf{Max-Set}      & 38.38±1.57 & 95.94±0.52           & 92.19±0.47          &84.84±0.48 & 42.52±1.32          & \textbf{47.13±5.18} & 52.22±0.94              & 90.22±0.51          & 95.42±0.51          & \textbf{86.09±0.48} \\
      \bottomrule[1pt]
    \end{tabular}
  }
  \label{tab:nrl-f}
\end{table*}


==> tabs/nrl.tex <==

\begin{table}[t]
    \centering
    \caption{Abalation of \NRL funtions.}
    \renewcommand{\arraystretch}{1.1}
    \resizebox{\columnwidth}{!}{
    \begin{tabular}{l|lllll}
    \toprule[1pt]
        \textbf{\NRL} & \textbf{Actor} & \textbf{squirrel} & \textbf{chameleon} & \textbf{pubmed} \\ 
        \midrule[0.8pt]

      \textbf{None}     & 36.76±1.00          & 42.13±1.99          & 44.66±3.46           & 90.29±0.50           \\
      \textbf{Concat}   & 37.95±1.89          & \textbf{43.42±1.66} & 44.33±4.57           & 90.23±0.50           \\
      \textbf{LSTM}     & 37.20±1.27          & 41.21±2.84          & 46.52±3.46           & 90.27±0.72           \\
      \textbf{Mean}     & 37.54±1.96          & 42.81±1.73          & 44.55±5.04           & \textbf{90.38±0.42}  \\
      \textbf{Sum}      & 37.76±1.92          & 43.26±1.86          & 45.39±4.25           & 90.25±0.43           \\
      \textbf{Max}      & \textbf{38.38±1.57} & 42.52±1.32          & \textbf{47.13±5.18}  & 90.22±0.51           \\
        
        \bottomrule[1pt]
    \end{tabular}
    }
\label{tab:nrl}
\end{table}



==> tabs/nst.tex <==

\begin{table}[t]
    \centering
    \caption{Abalation of Three Principles. }
    \renewcommand{\arraystretch}{1.1}
    \resizebox{\columnwidth}{!}{
    \begin{tabular}{lll|lllll}
    \toprule[1pt]
        \multicolumn{3}{c|}{\textbf{FlatGCN}}  & \multirow{2}{*}{\textbf{Flickr}}&\multirow{2}{*}{\textbf{squirrel}} & \multirow{2}{*}{\textbf{chameleon}} & \multirow{2}{*}{\textbf{pubmed}} \\ 
        \textbf{\SN} & \textbf{\IN} & \textbf{\RN}  &  &  & \\ 
        \midrule[0.8pt]

        &  &   & 65.65±1.34& 37.06±1.42 & 41.46±3.42 & 87.70±0.58\\ 
       \checkmark  &  &    & & & & \\ 
         & \checkmark &   & & & & \\ 
         &  & \checkmark  & & & & \\ 
       \checkmark  &  &  \checkmark  & & & & \\ 
       \checkmark  & \checkmark &    & & & & \\ 
         & \checkmark &  \checkmark  & & & & \\ 
       \checkmark  & \checkmark &  \checkmark  & & & & \\ 
        
        \bottomrule[1pt]
    \end{tabular}
    }
\label{tab:nst}
\end{table}
